Reducing health and climate impacts of the global food system

The global food system contributes to tens of millions of years of human life lost every year through unhealthy diets, and accounts for roughly a third of greenhouse gas (GHG) emissions. Researchers have thus often sought opportunities to simultaneously redress these large impacts on human health and climate; "dietary shifts" are frequently identified as key to both improving health and reducing land-related GHG emissions. Here we develop a new, spatially-explicit, detailed model of the global food system, and use it to highlight enormous and low-cost opportunities to both improve dietary health and reduce food system emissions. However, we find that health and climate goals are surprisingly independent; for example, reducing red meat intake benefits climate, but may only modestly improve health outcomes. Similarly, there is very large potential both to achieve healthier diets that do not lead to emissions reductions and to reduce emissions without dietary change. Our results highlight both the potential for, and the separability of, food-related policies that advance public health and climate goals.

==> manuscript_numbers/numbers.tex <==
% Auto-generated by scripts/transition_numbers.py — do not edit by hand.
% Re-run ``snakemake transition_numbers`` to refresh.
% Macros expand to bare numbers; wrap in siunitx (e.g. \qty{\macro}{Mha}).

\newcommand{\centralGhgPrice         }{50} % USD/tCO2eq
\newcommand{\centralYllValue         }{5000} % USD/YLL
\newcommand{\croplandRef             }{1400} % Mha (2 sf)
\newcommand{\croplandCentral         }{1400} % Mha (2 sf)
\newcommand{\grasslandRef            }{2300} % Mha (2 sf)
\newcommand{\grasslandCentral        }{1600} % Mha (2 sf)
\newcommand{\croplandReducPct        }{1} % %
\newcommand{\grasslandReducPct       }{29} % %
\newcommand{\landSavedGha            }{0.7} % Gha
\newcommand{\tradedLandMha           }{710} % Mha (2 sf)
\newcommand{\tradedLandPctAg         }{19} % %
\newcommand{\netEmRef                }{5.5} % GtCO2eq/yr
\newcommand{\netEmCentral            }{-0.9} % GtCO2eq/yr
\newcommand{\emAvoided               }{6.4} % GtCO2eq/yr
\newcommand{\seqCentral              }{-6.7} % GtCO2eq/yr
\newcommand{\seqCentralAbs           }{6.7} % GtCO2eq/yr (magnitude)
\newcommand{\directEmRef             }{6.4} % GtCO2eq/yr (CH4+N2O)
\newcommand{\landSinkRef             }{1.0} % GtCO2eq/yr (baseline sink)
\newcommand{\yllRef                  }{70} % MYLL/yr
\newcommand{\yllCentral              }{26.5} % MYLL/yr
\newcommand{\yllAvoided              }{44} % MYLL/yr
\newcommand{\yllReducPct             }{62} % %
\newcommand{\prodCostRef             }{3400} % bnUSD/yr (2 sf)
\newcommand{\prodCostCentral         }{3100} % bnUSD/yr (2 sf)
\newcommand{\prodCostSavings         }{290} % bnUSD/yr (2 sf)
\newcommand{\prodCostReducPct        }{9} % %
\newcommand{\consumerSurplusLoss     }{280} % bnUSD/yr (2 sf)
\newcommand{\yllCeilingHighVal       }{26} % MYLL (rounded up to 2 sf)
\newcommand{\yllSynergyLowGhg        }{57} % MYLL/yr (low GHG, low YLL slice)
\newcommand{\yllSynergyHighGhg       }{47} % MYLL/yr (high GHG, low YLL slice)
\newcommand{\ghgConditionalStdMax    }{4.5} % GtCO2eq
\newcommand{\netZeroGhgLo            }{26} % USD/tCO2eq
\newcommand{\netZeroGhgHi            }{37} % USD/tCO2eq
\newcommand{\netZeroGhgFlex          }{35} % USD/tCO2eq (flexible diet)
\newcommand{\netZeroGhgFixed         }{70} % USD/tCO2eq (fixed diet)
\newcommand{\netZeroGhgFixedVsFlexPct}{101} % % (fixed vs. flexible net-zero price)
\newcommand{\highGhgThreshold        }{200} % USD/tCO2eq
\newcommand{\highGhgEmCeilingAbs     }{6} % GtCO2eq/yr (abs)
\newcommand{\highGhgRefPrice         }{500} % USD/tCO2eq
\newcommand{\lowGhgRefPrice          }{5} % USD/tCO2eq
\newcommand{\emFlexHighGhg           }{-8} % GtCO2eq/yr
\newcommand{\emFixedHighGhg          }{-4} % GtCO2eq/yr
\newcommand{\emAbatedFlexHighGhg     }{12} % GtCO2eq/yr abated
\newcommand{\emAbatedFixedHighGhg    }{9} % GtCO2eq/yr abated
\newcommand{\feedLowGhg              }{6700} % Mt dry matter (2 sf)
\newcommand{\feedHighGhg             }{5500} % Mt dry matter (2 sf)
\newcommand{\fcrRumLowGhg            }{370} % kg DM / kg protein (2 sf)
\newcommand{\fcrRumHighGhg           }{280} % kg DM / kg protein (2 sf)
\newcommand{\croplandReleasedCentral }{11} % Mha (2 sf)
\newcommand{\pastureReleasedCentral  }{650} % Mha (2 sf)
\newcommand{\pastureReleasedBraMha   }{95} % Mha
\newcommand{\croplandReleasedBraMha  }{1} % Mha
\newcommand{\reforestedBraPctOwnAg   }{38} % %
\newcommand{\reforestedBraTotalMha   }{95} % Mha (2 sf)
\newcommand{\reforestedChnPctOwnAg   }{28} % %
\newcommand{\reforestedChnTotalMha   }{120} % Mha (2 sf)
\newcommand{\numCrops                }{48} % count
\newcommand{\numFoods                }{68} % count
\newcommand{\exogForageGtdm          }{0.3} % Gt DM/yr
\newcommand{\exogForageCountries     }{14} % count
\newcommand{\exogForageTopFivePct    }{88} % %
\newcommand{\devLambdaC              }{1.56} % bnUSD/Mha
\newcommand{\devLambdaP              }{0.16} % bnUSD/Mha
\newcommand{\devLambdaA              }{0.07} % bnUSD/MtDM
\newcommand{\devCroplandPct          }{5.01} % %
\newcommand{\devPasturePct           }{5.00} % %
\newcommand{\devFeedPct              }{4.92} % %
\newcommand{\valLandSlackMha         }{0.04} % Mha
\newcommand{\valFoodSlackMt          }{99} % Mt
\newcommand{\valFoodDemandMt         }{4108} % Mt
\newcommand{\valFoodSlackPct         }{2.4} % %
\newcommand{\valDairySlackMt         }{22} % Mt
\newcommand{\valDairySlackOfDemandPct}{2.3} % %
\newcommand{\valVegSlackMt           }{32} % Mt
\newcommand{\valFruitSlackMt         }{21} % Mt

